Dynamic loss balancing and sequential enhancement for road-safety assessment and traffic scene classification

Road-safety inspection is an indispensable instrument for reducing road-accident fatalities contributed to road infrastructure. Recent work formalizes road-safety assessment in terms of carefully selected risk factors that are also known as road-safety attributes. In current practice, these attributes are manually annotated in geo-referenced monocular video for each road segment. We propose to reduce dependency on tedious human labor by automating recognition with a two-stage neural architecture. The first stage predicts more than forty road-safety attributes by observing a local spatio-temporal context. Our design leverages an efficient convolutional pipeline, which benefits from pre-training on semantic segmentation of street scenes. The second stage enhances predictions through sequential integration across a larger temporal window. Our design leverages per-attribute instances of a lightweight bidirectional LSTM architecture. Both stages alleviate extreme class imbalance by incorporating a multi-task variant of recall-based dynamic loss weighting. We perform experiments on the iRAP-BH dataset, which involves fully labeled geo-referenced video along 2,300 km of public roads in Bosnia and Herzegovina. We also validate our approach by comparing it with the related work on two road-scene classification datasets from the literature: Honda Scenes and FM3m. Experimental evaluation confirms the value of our contributions on all three datasets.

==> figures/figure_04.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.95\textwidth]{img/grid_examples.jpg}
    \caption{
Qualitative experiments on iRAP-BH for 5 road-safety attributes.
For each attribute, the top row shows 5 input images
with the groundtruth label, while the bottom row presents
the corresponding saliency maps and the predictions
 of the two stages of our model (conv, seq). 
     }
    \label{fig:appendix_examples}
\end{figure*}
